Parameterized Model-checking of Discrete-Timed Networks and Symmetric-Broadcast Systems

We study the complexity of the model-checking problem for parameterized discrete-timed systems with arbitrarily many anonymous and identical processes, with and without a distinguished "controller", and communicating via synchronous rendezvous. Our framework extends the seminal work from German and Sistla on untimed systems by adding discrete-time clocks to processes. For the case without a controller, we show that the systems can be efficiently simulated -- and vice versa -- by systems of untimed processes that communicate via rendezvous and symmetric broadcast, which we call "RB-systems". Symmetric broadcast is a novel communication primitive that allows all processes to synchronize at once; however, it does not distinguish between sending and receiving processes. We show that the parameterized model-checking problem for safety specifications is pspace-complete, and for liveness specifications it is decidable in exptime. The latter result is proved using automata theory, rational linear programming, and geometric reasoning for solving certain reachability questions in a new variant of vector addition systems called "vector rendezvous systems". We believe these proof techniques are of independent interest and will be useful in solving related problems. For the case with a controller, we show that the parameterized model-checking problems for RB-systems and systems with asymmetric broadcast as a primitive are inter-reducible. This allows us to prove that for discrete timed-networks with a controller the parameterized model-checking problem is undecidable for liveness specifications. Our work exploits the intimate connection between parameterized discrete-timed systems and systems of processes communicating via broadcast, providing a rare and surprising decidability result for liveness properties of parameterized timed-systems, as well as extend work from untimed systems to timed systems.

==> figures/ex_dtn.tex <==

\subsection{Solving PMCP for Specifications over Finite Executions}\label{sec: PMCP finite}

We can now address the PMCP for specifications given in the form of nondeterministic finite automata, and show that the problem is \PSPACE-complete.
We do this using the automata theoretic approach. In particular, given an RB-template $\proctemp$ be build an NFW $\execNFW$ that accepting exactly the executions in $\execfin$. Intuitively, $\execNFW$ is just the reachability-unwinding $\puwd$ viewed as an automaton. Model checking of a regular specification given by an NFW $\A'$ is thus reduced to checking language containment of $\execNFW$ in $\A'$.

Here is the construction. 
\begin{definition} \label{dfn: automaton for finite executions}
Given an RB-template $\proctemp = \tup{\AP,\Actionprts \cup \{\brd\}, S,I,R,\lambda}$, consider the reachability-unwinding $\puwd = \tup{AP,\Actionprts \cup \{\brd\},S^\uwd,I^\uwd,R^\uwd,\lambda^\uwd}$. 
Define $\execNFW$ to be the NFW $\tup{\Sigma,S',I',R',F}$ with input alphabet $\Sigma = 2^{AP}$, state set $S' = S^\uwd$, initial-states set $I' = I^\uwd$, transition relation $R'$ consisting of transitions $(s,\lambda^\uwd(t),t)$ for $(s,\sigma,t) \in R^\uwd$, and final-states set $F = S^\uwd$.  
\end{definition}

The fact that words accepted by $\execNFW$ are exactly the executions in $\execfin$ is an immediate consequence of Proposition~\ref{prop: unwinding captures executions}. Analysing the construction of the unwinding template $\puwd$ in Section~\ref{sec: unwinding}, we get that $\execNFW$ is of size at most exponential in the size of $\proctemp$. 


% given a process template $\proctemp$.
%The automaton $\execNFW$ also serves as the starting point of the construction in Section~\ref{sec: b-automaton construction}.

% \begin{lemma} \label{lem: automaton for finite executions}
%  The size of $\execNFW$ is at most exponential in the size of $\proctemp$, and accepts exactly the executions in $\execfin$.
% \end{lemma}
% \begin{proof}
% Let $\proctemp = \tup{AP,\Actionprts \cup \{\brd\}, S,I,R,\lambda}$ be a process template.
% We show how to build an NFW $\execNFW$ whose language is $\execfin$.
% Model checking of a regular specification given by an NFW $\A'$ is thus reduced to checking language containment of $\execNFW$ in $\A'$.
% 
% % \srcomment{i introduced a fresh initial state, and labeled an edge of the automaton by the label of its target, not source}
% 
% Intuitively, the NFW $\execNFW$ is the reachability-unwinding $\puwd$ viewed as an automaton, with a fresh initial state and all other states being accepting.
% Formally, given $\puwd = \tup{AP,\Actionprts \cup \{\brd\},S^\uwd,I^\uwd,R^\uwd,\lambda^\uwd}$, define
%  $\execNFW$ to be the tuple
%  \[
%   \tup{2^{AP},S^\uwd \cup \{init\},\{init\},\delta,S^\uwd}
%  \]
% where $init$ is a fresh state, and $\delta$ consists of the transitions $(init,\lambda^\uwd(s),s)$ for $s \in I^\uwd$, as well as $(s,\lambda^\uwd(t),t)$ for $(s,\sigma,t) \in R^\uwd$.
% % \srcomment{the previous version wrote $(s,i)$ and $(t,i)$ instead of $s$ and $t$. is that better?}
% The fact that words accepted by $\execNFW$ are exactly the executions in $\execfin$ is an immediate consequence of Proposition~\ref{prop: unwinding captures executions}.
% 
% Analysing the construction of the unwinding template $\puwd$ in Section~\ref{sec: unwinding}, we get that $\execNFW$ is of size at most exponential in the size of $\proctemp$. \qed
% \end{proof}


\begin{theorem}\label{thm: finite RB PMCP is in pspace}
  The PMCP of RB-systems for regular specifications is in \PSPACE.
  %if constants in the guards are coded in unary)
\end{theorem}
\begin{proof}
Let $\proctemp = \tup{\AP,\Actionprts \cup \{\brd\}, S,I,R,\lambda}$ be a process template, and let $\execNFW$ be the NFW from Definition~\ref{dfn: automaton for finite executions}.

We describe a \PSPACE\ algorithm for checking the containment of the language accepted by $\execNFW$ in the language of some specification NFW $\A'$. This is done by solving the non-containment problem in nondeterministic polynomial space, and using the fact that \NPSPACE\ = \PSPACE\ = co-\PSPACE.
The algorithm constructs on the fly: (1) a finite word $\rho \in 2^\AP$, and an accepting run of $\execNFW$ on $\rho$; and (2) checks that $\rho$ is not accepted by $\A'$.
Item (2) can be done, as usual, simply by storing the subset of states of $\A'$ that are reachable by reading the prefix of $\rho$ constructed thus far, and validating that, at the end, this set does not contain an accepting state.
For item (1), the algorithm does not store all of (the exponentially big $\execNFW$). Instead, at each point in time, it only stores a single component $\puwd_i$ of $\puwd$ (which can be calculated in \PTIME for every $i$), from which it can deduce the part of $\execNFW$ corresponding to it. The algorithm starts by constructing $\puwd_0$, and sets $\rho$ to be the empty word, and the run of $\execNFW$ on $\rho$ to be the initial state of $\execNFW$. At each step, it can either declare the guess as finished (if the run constructed thus far ends in an accepting state of $\execNFW$) or extend $\rho$ and the run. Extending $\rho$ is a trivial guess. Extending the guessed run is done by either guessing a transition of $\execNFW$ inside  the component induced by the currently stored $\puwd_i$; or by guessing a transition that moves to the next component in the lasso, at which point the algorithm also discards $\puwd_i$ and replaces it with $\puwd_{\comp(i)}$.
%The result on the PMCP of timed networks now follows from Lemma~\ref{lem:timed-networks-limited}.
\qed
\end{proof}

In the next theorem we state a corresponding lower bound.
Interestingly, our proof shows that the problem is already  \PSPACE\ hard for \emph{reachability} specifications.

% \sr{SR and BA to check correctness and shorten}


% \sr{sketch of lower bound for BPs: reduce QBF to BP. for the kernel, assume it is in CNF. disjuncts are nested if then else. conjuncts are sequences of these.
% for the quantifiers, think of each quantifier as a function that calls the next quantifier with one of two values. note, that each function is called in exactly two places. so for each quantifier, we add a boolean variable that tells where to return to.}

\begin{theorem}\label{thm: lower-bound-finite-PMCP}
  The PMCP of RB-systems for regular specifications is \PSPACE-hard.
\end{theorem}
\begin{proof}
% \ba{@FS, please replace occurrences of $k$ for the number of variables with anoither letter (we use $k$ to denote the number of processes in a rendezvous)}
  The proof proceeds by a reduction from the reachability problem for Boolean programs, known to be \PSPACE-complete~\cite{books/daglib/0090683}.

  A Boolean program consists of $m$ Boolean variables $X_1, \ldots, X_m$ (for some $m$) and $n$ instructions (for some $n$), referred to by their \emph{program location} $l \in [n]$, of two types: \emph{(i)} \emph{conditionals} of the form $l: \texttt{if } X_i  \texttt{ then } l_{if}  \texttt{ else } l_{else}$; \emph{(ii)} \emph{toggles} of the form $l: X_i := \neg X_i$. The semantics of the first type of instruction is to move from location $l$ to location $l_{if}$ if $X_i$ is true and to location $l_{else}$ otherwise; instructions of this type are thus conditional jumps that do not change the values of any of the Boolean variables.
  The semantics of the second type of instruction is to negate the value of the Boolean variable $X_i$;
  %; the values of the other Boolean variables are left unchanged;
  the execution continues from location $l+1$ (unless that was the last instruction). We let $var(l)$ denote the index $i$ of the variable used (i.e., tested or toggled) in the instruction in program location $l$.
  All Boolean variables are initialized to $\texttt{false}$ and execution begins with instruction $1$.
  We remark that the Boolean programs considered here are deterministic.
  The reachability problem for Boolean programs is to decide whether the execution of a Boolean program ever reaches its last instruction.  Note that we can assume, without loss of generality, that the last instruction of a Boolean program is a conditional instruction.

  Given a Boolean program $B$, we build a process template $P$, and a specification formula $\varphi$, such that
  $\psys$ satisifes $\varphi$ iff the execution of $B$ reaches its last instruction.

  Formally, $\proctemp = \tup{AP,\Actionprts \cup \{\brd\}, S,\{\iota\},R,\lambda}$, where:
  \begin{itemize}
    \item $AP = [n]$;
    \item $\Actionprts = \cup_{\msg{a} \in \Actions} \{ \msg{a}_1, \msg{a}_2\}$  where
    $\Actions = \cup_{i \in [m]} \{ \msg{(\text{protect},i)}, \msg{(\text{if},i)}, \msg{(\text{else},i)}, \msg{(\text{toggle},i)} \}$;

    \item The set of states $S := \{\iota, \tt{sink}\} \cup S_{instr} \cup S_{var}$, where $\iota$ is an initial state, $\tt{sink}$ is a sink state, and:
    \begin{enumerate}
        \item $S_{var} := \cup_{i \in [m]} \{X_i, \neg X_i, X'_i, \neg X'_i\}$,
        \item $S_{instr} := \cup_{l \in [n]} \{l,l'\}$, 
    \end{enumerate}
    \item $R$ will be defined later;
    \item the labeling relation $\lambda$ contains all pairs of the form $(l, l)$ for $l \in [n]$. \srcomment{add $\Box$ for the labeling the other states}
%     \fz{This labelling function misses states that do not simulate locations.} \srcomment{$\lambda$ is a relation, not a function. or do you mean that the semantics is wrong somehow?}
  \end{itemize}

  The specification formula $\varphi$ says that the last program location is never visited. This can be expressed, for instance, by the regular expression $(\Box + [n-1])^*$. 
%   \fz{Similarly, the specification does not deals with states that are not locations.}

  Before describing the transition relation $R$, we briefly describe the way the states are used in the simulation of the Boolean program $B$  by runs of $\psys$.
%
  At the beginning of every run, every process nondeterministically moves (on a broadcast) from the initial state either to the state $1$, or to one of the states $\neg X_1, \cdots, \neg X_m$. A process that moves to the state $1$ will keep track of (i.e., encode) the program location of the Boolean program, and from this point on will only be in states from the set $S_{instr}$; whereas a process that moves to a state of the form $\neg X_i$ will keep track of (i.e., encode) the value of variable $X_i$, and from this point on will only be in states from the set $\{X_i, \neg X_i, X'_i, \neg X'_i\}$. Observe that multiple processes may decide to encode the program location or the same variable. However,
  the transition relation $R$ will be defined in such a way as to enforce the invariant that, right after every broadcast, the following holds: $(\dagger)$ all processes that encode the same object (i.e., the program location or the value of some variable) agree on its value. Moreover, between every two broadcasts, at most one instruction of the Boolean program can be simulated, namely, the instruction referenced by the processes that track the program location. The primed versions of the states will be used in order to enforce this round structure, as well as the invariant $\dagger$, as follows: in each round, every rendezvous transition moves a process from an unprimed state to a primed state, from which it can only move on a broadcast; whereas a broadcast takes a process in a primed state back to an unprimed state, and processes in an unprimed state to $\tt{sink}$.

  We now define the transition function $R$ of the template $\proctemp$. It consists of the following transitions:
\begin{itemize}
\item $\trans{\iota}{1}{\brd}$; $\trans{\iota}{\neg X_i}{\brd}$ for $i \in [m]$,
\item $\trans{\tt{sink}}{\tt{sink}}{\brd}$; $\trans{l}{\tt{sink}}{\brd}$,  $\trans{X_i}{\tt{sink}}{\brd}$, $\trans{\neg X_i}{\tt{sink}}{\brd}$, for $l \in [n], i \in [m]$,
\item $\trans{l'}{l}{\brd}$, $\trans{X'_i}{X_i}{\brd}$, and $\trans{\neg X'_i}{\neg X_i}{\brd}$.

\item $\trans{l}{l}{\msg{(\text{protect},i)}_1}$ for $l \in [n]$ and $i \in [n] \setminus var(l)$.  \srcomment{recall what is var}
\item $\trans{X_i}{X'_i}{\msg{(\text{protect},i)}_2}$ and
$\trans{\neg X_i}{\neg X'_i}{\msg{(\text{protect},i)}_2}$ for $i \in [m]$.
\item $\trans{l}{l'_{if}}{\msg{(\text{if},var(l))}_1}$ and $\trans{l}{l'_{else}}{\msg{(\text{else},var(l))}_1}$ for all conditional instructions $l$.
\item $\trans{X_i}{X'_i}{\msg{(\text{if},i)}_2}$ and $\trans{\neg X_i}{\neg X'_i}{\msg{(\text{else},i)}_2}$ for $i \in [m]$.
\item $\trans{l}{(l+1)'}{\msg{(\text{toggle},var(l))}_1}$ for all toggle instructions $l$.
\item $\trans{X_i}{\neg X'_i}{\msg{(\text{toggle},i)}_2}$ and $\trans{\neg X_i}{X'_i}{\msg{(\text{toggle},i)}_2}$ for $i \in [m]$.
\end{itemize}
% \fz{The function $var(l)$ is not defined so far. Further, the function is used with different fonts, which is confusing.}
% \srcomment{var was defined at the start of the proof.}
% \srcomment{i've tried to improve the fonts}

We now prove that the reduction is correct.

Suppose that the infinite run $\rho$ of the Boolean program visits its last instruction. We build a run $\pi$ of $\sysinst{m+1}$ witnessing the fact that
$\psys$ does not satisfy $\varphi$. The run $\pi$ simulates $\rho$ as follows. Start with a broadcast, which takes process $m+1$ (called the \emph{controller process}) to state $1$, and for every $i \in [m]$ takes process $i$ (called the \emph{$i$th variable process}) to $\neg X_i$.
Repeatedly extend the run $\pi$ by the following sequence of global transitions (below, $l$ denotes the current state of the controller process):
\begin{enumerate}
 \item For every $i \neq var(l)$, the controller rendezvous with the $i$th memory process on the action $\msg{(\text{protect},i)}$.
 \item The controller rendezvous with the $var(l)$th memory process as follows: if $l$ is a toggle instruction then the rendezvous action is $\msg{(\text{toggle},i)}$; otherwise, it is $\msg{(\text{if},i)}$ if the $i$th memory process is in state $X_i$, and it is $\msg{(\text{else},i)}$ if it is in state $\neg X_i$.
 \item A broadcast.
\end{enumerate}

It is easy to see that $\pi$ simulates $\rho$. In particular, the state of the controller after $k \geq 1$ broadcasts is equal to the program location of the Boolean program after $k$ steps.


For the other direction, we argue as follows. We say that a configuration $f$ of $\psys$ is \emph{consistent} if it satisfies the invariant $\dagger$ stated earlier. For such an $f$, let $pl(f) \in [n]$ be the program location encoded by $f$, or $\bot$ if there are no processes in $f$ tracking the program location; and for every $i \in [m]$, let $val_i(f) \in \{\true, \false\}$ be the value of $X_i$ encoded by $f$, or $\bot$ if there are no processes in $f$ tracking the value of $X_i$. Given $k \in \mathbb{N}$, and a run $\pi$ of $\psys$ with at least $k$ broadcasts, write $\pi(k)$ for the configuration in $\pi$ immediately following the $k$th broadcast. Observe that it is enough to show that $\pi$ simulates the run $\rho$ of the Boolean program in the following sense:
\begin{enumerate}
 \item $\pi(k)$ is consistent,
 \item if $pl(f_k) \neq \bot$ then the program location in $\rho_k$ is equal to $pl(f_k)$,
 \item for every $i \in [m]$, if $val_i(f_k) \neq \bot$ then the value of variable $X_i$ in $\rho_k$ is equal to $val_i(f_k)$.
\end{enumerate}

We prove the items above by induction on $k$. For $k = 1$, i.e., after the first broadcast (which must be the first transition on any run), processes assume different roles. Any process that moves to state $1$ is called a \emph{controller}, and
any process that moves to state $\neg X_i$ (for some $i \in [m]$) is called an \emph{$i$th variable processes}. Clearly the induction hypothesis holds. For the inductive step, note that by the inductive hypothesis $\pi(k-1)$ is consistent, let $l := pl(\pi(k-1))$, and observe that the only rendezvous transitions on $\pi$ between the $k-1$ and $k$ broadcasts are of a controller process that rendezvous with a variable process on an action of the form described in items $1$ and $2$ in the proof of the first direction (in particular, if $l = \bot$ then there are no rendezvous between the $k-1$ and $k$ broadcasts). Thus, it must be that, just before the $k$th broadcast, processes in a primed state that are encoding the same object are in the same state. Combining this with the fact that any process in an unprimed state will move to $\tt{sink}$ on the $k$th broadcast one can see that the inductive hypothesis holds also after the $k$th broadcast.   \qed
%
%   \sr{...and  how they are used to simulate the instructions of a Boolean program.}
%   For every instruction of the form $l: \texttt{if } X_i  \texttt{ then } l_1  \texttt{ else } l_2$
%   \ba{@FS, can you please continue by giving a more formal definition of the transitions, as well as polish (make more formal where needed, etc.) the rest of the proof?}
%   we have four two transitions: one which takes a process from each of the states $(X_i = \texttt{true})$ and $(\texttt{Inst} = l)$ to the states $(X_i = \texttt{true})'$ and $(\texttt{Inst} = l_1)'$ respectively, and one which takes a process from each of the states $(X_i = \texttt{false})$ and $(\texttt{Inst} = l)$ to the states $(X_i = \texttt{false})'$ and $(\texttt{Inst} = l_2)'$.
%   For $l: X_i := \neg X_i$, we have two rendezvous transitions, one transition which takes a process from each of the states  $(X_i = \texttt{true})$ and $(\texttt{Inst} = l)$ and moves them to the states $(X_i = \texttt{false})'$ and $(\texttt{Inst} = l+1)'$, and one transition which takes a process from each of the states  $(X_i = \texttt{false})$ and $(\texttt{Inst} = l)$ and moves them to the states $(X_i = \texttt{true})'$ and $(\texttt{Inst} = l+1)'$.
%   Additionally we need rendezvous transitions which allow the Boolean variables that do not appear in the simulated instruction to keep the same value, and not sink in the next broadcast:
%   For both instructions we further have two rendezvous transitions for each variable $X_j \neq X_i$, one transition which takes a process
%   from each of the states $(X_j = \texttt{true})$ and $(\texttt{Inst} = l)$ and moves them to the states $(X_j = \texttt{true})'$ and $(\texttt{Inst} = l)$, and one transition which takes a process from each of the states $(X_j = \texttt{false})$ and $(\texttt{Inst} = l)$ and moves them to the states $(X_j = \texttt{false})'$ and $(\texttt{Inst} = l)$;
%   we note that these rendezvous transitions do not move the process in state $(\texttt{Inst} = l)$ to a primed state in order to allow all variables $X_j \neq X_i$ to be moved to a primed state;
%   only the earlier described rendezvous transitions move a process in state $(\texttt{Inst} = l)$ to a primed state.
%   It remains to describe the broadcast transition of the process template.
%   The broadcast transition moves all processes in primed states to the corresponding unprimed state and all processes in an unprimed state to the sink state $\tt{sink}$ from which processes cannot move any further;
%   further, the broadcast transition moves all processes in the initial state $\iota$ to some of the states $(X_i = \texttt{false})$ and $(\texttt{Inst} = 1)$.
%
%   We now describe the properties of the constructed process template.
%   We claim that (1) the process template can simulate the execution of the Boolean program and (2) all runs of the process template need to follow the execution of the Boolean program.
%
%   For (1), we assume an instantiation of the process template with $k+1$ processes (where $k$ is the number of variables of the Boolean program).
%   Then, an initial broadcast can move exactly one process to each of the states $(X_i = \texttt{false})$ and $(\texttt{Inst} = 1)$.
%   Now, the instructions of the Boolean program are simulated in rounds.
%   In each round, first only rendezvous transitions are taken.
%   Then, one broadcast is taken to close the round.
%   For $l: \texttt{if } X_i  \texttt{ then } l_1  \texttt{ else } l_2$,
%   the rendezvous transitions first move all the variables $X_j \neq X_i$ to the corresponding primed state with the same value;
%   then the rendezvous transition is applied which checks $X_i$ and moves to the next instruction.
%   For $l: X_i := \neg X_i$,
%   the rendezvous transitions first move all the variables $X_j \neq X_i$ to the corresponding primed state with the same value;
%   then the rendezvous transition is applied which flips the value of $X_i$.
%   We observe that in this way an execution of a Boolean program can be simulated by $k+1$ processes which mimic the state of the Boolean program by having one process in a state for each variable $X_i$ and one process in state $(\texttt{Inst} = l)$ for the current instruction $l$.
%
%   For (2), we observe that the construction of the process ensures the invariant that that processes can be at most in one of the states $(X_i= \texttt{false})$ or $(X_i = \texttt{true})$ and at most in one of the states $(\texttt{Inst} = l)$ for $l \in [1,n]$.
%   (We note that there can be many processes in each of the states because of the loading property, but this is not important for construction, we only care about the mutual exclusion property we stated).
%   We point out that the invariant is ensured by the use of the primed states because rendezvous transitions always take processes from unprimed to primed states.
%   We further note that for each process there is exactly one rendezvous transition applicable which takes the process from an unprimed to a primed state.
%   Because of this property the processes in fact follow the run of the deterministic Boolean program.
%
%   We finally remark that our construction uses $k$-rendezvous transitions for $k=2$, i.e., the lower bound only relies on a fixed $k$.
\end{proof}

Theorems~\ref{thm: finite RB PMCP is in pspace} and \ref{thm: lower-bound-finite-PMCP} yield the following:

\begin{corollary}
    The PMCP of RB-systems for regular specifications is \PSPACE-complete.
\end{corollary}

\stable

\fz{12th March. Proof reading till here.}

\srcomment{12 May. Took most of Florian's comments into account.}

\textbf{Open Question:}\\
What is the complexity of deciding whether a rendezvous transition of an RB-system be taken infinitely often?

By Theorem~\ref{thm: lower-bound-finite-PMCP} above we have a \PSPACE\ lower bound (the proof can be used for the above question as well as we can introduce a self-loop in the Boolean program $\binstr{l}{\texttt{if } X_i  \texttt{ then } l  \texttt{ else } l}$ at the location of interest).
Our construction for deciding edge types gives an \textsc{exptime} upper bound.
It would be great to close this gap!


\fz{transfer lower bound to timed networks?}


%\sr{b: this would be PSPACE if we encode constants in guards in unary}

